Quantifying uncertainty in high-throughput density functional theory: a comparison of AFLOW, Materials Project, and OQMD

A central challenge in high throughput density functional theory (HT-DFT) calculations is selecting a combination of input parameters and post-processing techniques that can be used across all materials classes, while also managing accuracy-cost tradeoffs. To investigate the effects of these parameter choices, we consolidate three large HT-DFT databases: Automatic-FLOW (AFLOW), the Materials Project (MP), and the Open Quantum Materials Database (OQMD), and compare reported properties across each pair of databases for materials calculated using the same initial crystal structure. We find that HT-DFT formation energies and volumes are generally more reproducible than band gaps and total magnetizations; for instance, a notable fraction of records disagree on whether a material is metallic (up to 7%) or magnetic (up to 15%). The variance between calculated properties is as high as 0.105 eV/atom (median relative absolute difference, or MRAD, of 6%) for formation energy, 0.65 {\AA}$^3$/atom (MRAD of 4%) for volume, 0.21 eV (MRAD of 9%) for band gap, and 0.15 $\mu_{\rm B}$/formula unit (MRAD of 8%) for total magnetization, comparable to the differences between DFT and experiment. We trace some of the larger discrepancies to choices involving pseudopotentials, the DFT+U formalism, and elemental reference states, and argue that further standardization of HT-DFT would be beneficial to reproducibility.

==> multi-icsd-id-tables/across_db_comp_mm.tex <==
\\
\toprule
Databases & Compositions & ICSD UID \\
\midrule
\endfirsthead

\toprule
Databases & Compositions & ICSD UID \\
\midrule
\endhead

\multicolumn{3}{c}{Continued on the next page\ldots} \\
\bottomrule
\endfoot

\bottomrule
\endfoot

AFLOW-MP & \ce{Li2ScP2HO8}, \ce{Li2Sc(PO4)2} & 409955 \\
AFLOW-MP & \ce{Tl3HS2O9}, \ce{Tl3S2O9} & 35358 \\
AFLOW-MP & \ce{DyCHO4}, \ce{DyCO4} & 245344-409351 \\
AFLOW-MP & \ce{Ba5Re3O17}, \ce{Ba5Re3O16} & 100777 \\
AFLOW-MP & \ce{LiZnBi}, \ce{ZnBi} & 100115 \\
AFLOW-MP & \ce{RbOs2HO9}, \ce{RbOs2O9} & 20611 \\
AFLOW-MP & \ce{CdNHO4}, \ce{CdNO4} & 35355 \\
AFLOW-MP & \ce{Y3Fe31}, \ce{Y3Fe29} & 107259 \\
AFLOW-MP & \ce{Si2N3H}, \ce{Si2N3} & 202970 \\
AFLOW-MP & \ce{Y12(ReC3)5}, \ce{Y12Re5C6} & 658805 \\
AFLOW-MP & \ce{Na3VP2HO9}, \ce{Na3VP2O9} & 50760 \\
AFLOW-MP & \ce{YHO2}, \ce{YO2} & 28442 \\
AFLOW-MP & \ce{Dy2B3HO8}, \ce{Dy2B3O8} & 413927 \\
AFLOW-MP & \ce{LaHO2}, \ce{LaO2} & 60675 \\
AFLOW-MP & \ce{CdHOCl}, \ce{CdOCl} & 26752 \\
AFLOW-MP & \ce{HgHO4Cl}, \ce{HgO4Cl} & 29038 \\
AFLOW-MP & \ce{LiTa3(Bi2O7)2}, \ce{Ta3(Bi2O7)2} & 415141 \\
AFLOW-MP & \ce{NHTe2O7}, \ce{NTe2O7} & 14320-32608 \\
AFLOW-MP & \ce{HO3I}, \ce{O3I} & 26621 \\
AFLOW-MP & \ce{LiCH3O3}, \ce{LiCH2O3} & 109604 \\
AFLOW-MP & \ce{Ho2B3HO8}, \ce{Ho2B3O8} & 413928 \\
AFLOW-MP & \ce{Rb3H(SO4)2}, \ce{Rb3(SO4)2} & 60050 \\
AFLOW-MP & \ce{SrNH}, \ce{SrN} & 410656 \\
AFLOW-MP & \ce{SrHF3}, \ce{SrF3} & 35408 \\
AFLOW-MP & \ce{HgHO4Br}, \ce{HgO4Br} & 29039-31928 \\
AFLOW-MP & \ce{AlHO2}, \ce{AlO2} & 100390-100391-15696-27865-36340-59608-59609-59610-93728-93729-93730-93731-93732-93733-93734 \\
AFLOW-MP & \ce{C2NHS2(O2F3)2}, \ce{C2NS2(O2F3)2} & 50524 \\
AFLOW-MP & \ce{HoHO2}, \ce{HoO2} & 2944 \\
AFLOW-MP & \ce{Ca5P3HO13}, \ce{Ca5P3O13} & 16742-24240-81442 \\
AFLOW-MP & \ce{BaAl5HO9}, \ce{BaAl5O9} & 33282 \\
AFLOW-MP & \ce{RbHO}, \ce{Rb2O2} & 61048 \\
AFLOW-MP & \ce{KHO}, \ce{K2O2} & 61047-76958 \\
AFLOW-MP & \ce{MnP2HO7}, \ce{MnP2O7} & 415152 \\
AFLOW-MP & \ce{P3H(PbO5)2}, \ce{P3(PbO5)2} & 2494-71812 \\
AFLOW-MP & \ce{NdMoHO15I4}, \ce{NdMoO15I4} & 281173 \\
AFLOW-MP & \ce{PbHOCl}, \ce{PbOCl} & 27137-36267-76932 \\
AFLOW-MP & \ce{CaHOCl}, \ce{CaOCl} & 24403 \\
AFLOW-MP & \ce{La3TaH(O2Cl)3}, \ce{La3Ta(O2Cl)3} & 62189 \\
AFLOW-MP & \ce{LaNHO4}, \ce{LaNO4} & 413563 \\
AFLOW-MP & \ce{BaHF3}, \ce{BaF3} & 35409 \\
AFLOW-MP & \ce{Ga(Bi4O7)3}, \ce{Ga(Bi3O5)4} & 68648 \\
AFLOW-MP & \ce{XeSb2F10}, \ce{Xe2Sb4F19} & 157664 \\
AFLOW-MP & \ce{K2Cr2AsHO10}, \ce{K2Cr2AsO10} & 30533 \\
AFLOW-MP & \ce{H2O}, \ce{H7O4} & 27844 \\
AFLOW-MP & \ce{NdHO2}, \ce{NdO2} & 162390-162391 \\
AFLOW-MP & \ce{YCHO4}, \ce{YCO4} & 245345-644 \\
AFLOW-MP & \ce{KAl2P2H5O11}, \ce{KAl2P2H4O11} & 407355 \\
AFLOW-MP & \ce{Ta3Al4HO14}, \ce{Ta3Al4O14} & 67673 \\
AFLOW-MP & \ce{Ca2Al3Si3HO13}, \ce{Ca2Al3Si3O13} & 185684-185685-185686-185687-185688-185689-185690-185691-20235 \\
AFLOW-MP & \ce{SnPHO3}, \ce{SnPO3} & 25034 \\
AFLOW-MP & \ce{Ba5Cr3HO13}, \ce{Ba5Cr3O13} & 21034 \\
AFLOW-MP & \ce{Gd2CBr2}, \ce{GdBr} & 47226 \\
AFLOW-MP & \ce{CaCuAsHO5}, \ce{CaCuAsO5} & 64694 \\
AFLOW-MP & \ce{CuPbAsHO5}, \ce{CuPbAsO5} & 43455-54151 \\
AFLOW-MP & \ce{Ba5P3HO13}, \ce{Ba5P3O13} & 62283 \\
AFLOW-MP & \ce{Na3TiHF8}, \ce{Na3TiF8} & 14131 \\
AFLOW-MP & \ce{NdAl2}, \ce{Nd2Al} & 608745 \\
AFLOW-MP & \ce{NaCHO2}, \ce{NaCO2} & 109643 \\
\midrule
AFLOW-OQMD & \ce{Y3Fe31}, \ce{Y3Fe29} & 107259 \\
AFLOW-OQMD & \ce{LiB}, \ce{MnCoSiO4} & 2 \\
AFLOW-OQMD & \ce{Ga(Bi4O7)3}, \ce{Ga(Bi3O5)4} & 68648 \\
AFLOW-OQMD & \ce{H2O}, \ce{H7O4} & 27844 \\
\midrule
MP-OQMD & \ce{Bi3(PO5)2}, \ce{SmPd} & 107679 \\
MP-OQMD & \ce{SrGaH5}, \ce{SrGaH4} & 240697 \\
MP-OQMD & \ce{BaGaH5}, \ce{BaGaH4} & 240693 \\


==> multi-icsd-id-tables/outliers__band_gap.tex <==
\begin{tabular}{l l r r r c}
\toprule
Databases & Composition & $E_{\rm g}^1$ & $E_{\rm g}^2$ & $\Delta^{1-2}$ & ICSD UID \\
 & & \multicolumn{3}{c}{(eV)} & \\
\midrule
AFLOW-MP & \ce{CeF3} & $5.87$ & $0.00$ & $5.87$ & 42470 \\
AFLOW-MP & \ce{LiAlPHO5} & $0.02$ & $5.72$ & $-5.70$ & 68921 \\
AFLOW-MP & \ce{Na2PHO3} & $0.00$ & $5.58$ & $-5.58$ & 155976 \\
AFLOW-MP & \ce{KCeF4} & $5.44$ & $0.00$ & $5.44$ & 23229 \\
AFLOW-MP & \ce{RbYbF3} & $1.09$ & $6.52$ & $-5.43$ & 49590 \\
AFLOW-MP & \ce{K5NaCe2S6O24} & $5.49$ & $0.08$ & $5.41$ & 281576 \\
AFLOW-MP & \ce{CsYbF3} & $1.78$ & $7.05$ & $-5.26$ & 49579 \\
AFLOW-MP & \ce{BaTm2F8} & $1.97$ & $7.24$ & $-5.26$ & 20103 \\
AFLOW-MP & \ce{NaCeP2O7} & $5.26$ & $0.00$ & $5.26$ & 154075-416613 \\
AFLOW-MP & \ce{CePO4} & $5.23$ & $0.00$ & $5.23$ & 184550 \\
\midrule
AFLOW-OQMD & \ce{BeF2} & $8.04$ & $0.00$ & $8.04$ & 173557 \\
AFLOW-OQMD & \ce{LaF3} & $7.71$ & $0.00$ & $7.71$ & 246323-27089-35673 \\
AFLOW-OQMD & \ce{KYb3F10} & $0.97$ & $8.44$ & $-7.47$ & 28258 \\
AFLOW-OQMD & \ce{NaCaAlF6} & $7.12$ & $0.00$ & $7.12$ & 80542 \\
AFLOW-OQMD & \ce{H24OsC8N2F6} & $0.00$ & $6.68$ & $-6.68$ & 151185 \\
AFLOW-OQMD & \ce{YbCl3O12} & $0.00$ & $6.38$ & $-6.38$ & 85762 \\
AFLOW-OQMD & \ce{CoF2} & $6.30$ & $0.00$ & $6.30$ & 14144-26604-280604-53987-73460-9167-98785-98786 \\
AFLOW-OQMD & \ce{LiAlPHO5} & $0.02$ & $6.20$ & $-6.18$ & 68921 \\
AFLOW-OQMD & \ce{LiEuP4O12} & $0.33$ & $6.41$ & $-6.08$ & 416878 \\
AFLOW-OQMD & \ce{Na2PHO3} & $0.00$ & $6.07$ & $-6.07$ & 155976 \\
\midrule
MP-OQMD & \ce{KYb3F10} & $0.00$ & $8.44$ & $-8.44$ & 28258 \\
MP-OQMD & \ce{BeF2} & $7.96$ & $0.00$ & $7.96$ & 173557 \\
MP-OQMD & \ce{EuF2} & $0.00$ & $7.94$ & $-7.94$ & 238222-260882-29025 \\
MP-OQMD & \ce{KCeF4} & $0.00$ & $7.75$ & $-7.75$ & 23229 \\
MP-OQMD & \ce{H2} & $7.50$ & $0.00$ & $7.50$ & 28338-28340-638167 \\
MP-OQMD & \ce{NaCaAlF6} & $7.11$ & $0.00$ & $7.11$ & 80542 \\
MP-OQMD & \ce{EuMgF4} & $0.29$ & $7.22$ & $-6.94$ & 86246 \\
MP-OQMD & \ce{CsEuF3} & $0.00$ & $6.93$ & $-6.93$ & 49577 \\
MP-OQMD & \ce{H24OsC8(NF3)2} & $0.17$ & $6.68$ & $-6.51$ & 151185 \\
MP-OQMD & \ce{Yb(ClO4)3} & $0.00$ & $6.46$ & $-6.46$ & 85763 \\
\bottomrule
\end{tabular}


==> multi-icsd-id-tables/outliers__formation_energy_per_atom.tex <==
\begin{tabular}{l l r r r c}
\toprule
Databases & Composition & $\Delta E_{\rm f}^1$ & $\Delta E_{\rm f}^2$ & $\Delta^{1-2}$ & ICSD UID \\
 & & \multicolumn{3}{c}{(eV/atom)} & \\
\midrule
AFLOW-MP & \ce{AlPO4} & $-2.780$ & $-0.307$ & $-2.474$ & 162670 \\
AFLOW-MP & \ce{SiO2} & $-1.041$ & $-2.870$ & $1.829$ & 25632 \\
AFLOW-MP & \ce{Ho2Se3} & $-3.563$ & $-1.885$ & $-1.678$ & 408345-639705-639711 \\
AFLOW-MP & \ce{O} & $0.004$ & $1.669$ & $-1.665$ & 92775 \\
AFLOW-MP & \ce{C} & $0.004$ & $1.255$ & $-1.251$ & 88811-88815 \\
AFLOW-MP & \ce{NaAlSi3O8} & $-2.171$ & $-3.232$ & $1.061$ & 109006-171090-171091-171092-34870-34871-34872-68913-77421-77422-77423-77424-77425 \\
AFLOW-MP & \ce{AlClO} & $-1.741$ & $-2.789$ & $1.048$ & 27812 \\
AFLOW-MP & \ce{P2O5} & $-1.496$ & $-2.461$ & $0.966$ & 77377-82688 \\
AFLOW-MP & \ce{Bi} & $0.135$ & $1.090$ & $-0.954$ & 51675 \\
AFLOW-MP & \ce{SbAsO3} & $-0.765$ & $-1.719$ & $0.954$ & 37187-5286 \\
\midrule
AFLOW-OQMD & \ce{AlPO4} & $-2.780$ & $-0.237$ & $-2.543$ & 162670 \\
AFLOW-OQMD & \ce{Ho2Se3} & $-3.563$ & $-1.890$ & $-1.674$ & 408345-639705-639711 \\
AFLOW-OQMD & \ce{O} & $0.004$ & $1.395$ & $-1.391$ & 92775 \\
AFLOW-OQMD & \ce{MgO} & $-2.877$ & $-1.879$ & $-0.998$ & 181459 \\
AFLOW-OQMD & \ce{NaAlSi3O8} & $-2.171$ & $-3.053$ & $0.882$ & 109006-171090-171091-171092-34870-34871-34872-68913-77421-77422-77423-77424-77425 \\
AFLOW-OQMD & \ce{AlClO} & $-1.741$ & $-2.608$ & $0.867$ & 27812 \\
AFLOW-OQMD & \ce{P2O5} & $-1.496$ & $-2.303$ & $0.807$ & 77377-82688 \\
AFLOW-OQMD & \ce{RbC8} & $0.751$ & $-0.040$ & $0.791$ & 200563 \\
AFLOW-OQMD & \ce{SbAsO3} & $-0.765$ & $-1.524$ & $0.758$ & 37187-5286 \\
AFLOW-OQMD & \ce{K2BeO2} & $-1.259$ & $-2.002$ & $0.743$ & 23633 \\
\midrule
MP-OQMD & \ce{N2} & $0.000$ & $4.263$ & $-4.263$ & 638342-644518 \\
MP-OQMD & \ce{MnNiAs} & $3.547$ & $-0.249$ & $3.796$ & 161716 \\
MP-OQMD & \ce{Nd3PbN} & $-0.945$ & $1.319$ & $-2.264$ & 76397 \\
MP-OQMD & \ce{IrC4} & $0.981$ & $3.161$ & $-2.180$ & 181498 \\
MP-OQMD & \ce{Nd3SnN} & $-1.029$ & $1.112$ & $-2.141$ & 76398 \\
MP-OQMD & \ce{Sm3AlN} & $-0.894$ & $1.109$ & $-2.003$ & 52640 \\
MP-OQMD & \ce{LiNO3} & $0.690$ & $-1.252$ & $1.942$ & 33661 \\
MP-OQMD & \ce{Pr3AlN} & $-0.788$ & $1.101$ & $-1.888$ & 52639 \\
MP-OQMD & \ce{Cr3O} & $1.971$ & $0.141$ & $1.830$ & 15904 \\
MP-OQMD & \ce{Eu(Cu2Sn)2} & $1.296$ & $-0.322$ & $1.617$ & 416796 \\
\bottomrule
\end{tabular}


==> multi-icsd-id-tables/outliers__total_magnetization_per_atom.tex <==
\begin{tabular}{l l r r r c}
\toprule
Databases & Composition & $M^1$ & $M^2$ & $\Delta^{1-2}$ & ICSD UID \\
 & & \multicolumn{3}{c}{($\mu_{\rm B}$/formula unit)} & \\
\midrule
AFLOW-MP & \ce{YbMn28} & $124.89$ & $7.16$ & $117.72$ & 643923 \\
AFLOW-MP & \ce{Pr6Mn23} & $121.85$ & $32.42$ & $89.43$ & 643337 \\
AFLOW-MP & \ce{Tb6Mn23} & $101.04$ & $13.18$ & $87.86$ & 638317-643766-643774-643779 \\
AFLOW-MP & \ce{BaMn28} & $87.51$ & $8.61$ & $78.90$ & 615966 \\
AFLOW-MP & \ce{Yb6Mn23} & $105.23$ & $29.18$ & $76.05$ & 643920 \\
AFLOW-MP & \ce{Ba6Co25S27} & $66.99$ & $0.00$ & $66.99$ & 71939 \\
AFLOW-MP & \ce{Mn20W3C6} & $74.10$ & $16.64$ & $57.46$ & 618279 \\
AFLOW-MP & \ce{Mn20Mo3C6} & $73.37$ & $16.53$ & $56.84$ & 618260 \\
AFLOW-MP & \ce{Gd8Rh5C12} & $56.95$ & $0.15$ & $56.80$ & 617956 \\
AFLOW-MP & \ce{Nd12Co6Sn} & $56.33$ & $0.00$ & $56.33$ & 240094 \\
\midrule
AFLOW-OQMD & \ce{EuMn28} & $125.94$ & $4.13$ & $121.82$ & 631390 \\
AFLOW-OQMD & \ce{Gd13Ge6O31F} & $90.97$ & $0.01$ & $90.96$ & 62329 \\
AFLOW-OQMD & \ce{Pr6Mn23} & $121.85$ & $33.03$ & $88.82$ & 643337 \\
AFLOW-OQMD & \ce{BaMn28} & $87.51$ & $5.58$ & $81.93$ & 615966 \\
AFLOW-OQMD & \ce{Yb6Mn23} & $105.23$ & $30.78$ & $74.45$ & 643920 \\
AFLOW-OQMD & \ce{Ba6Co25S27} & $66.99$ & $2.23$ & $64.76$ & 71939 \\
AFLOW-OQMD & \ce{Nd12Co6Sn} & $56.33$ & $0.01$ & $56.32$ & 240094 \\
AFLOW-OQMD & \ce{Gd7Pd3} & $54.76$ & $0.89$ & $53.86$ & 104112 \\
AFLOW-OQMD & \ce{Gd7CoI12} & $51.02$ & $0.00$ & $51.01$ & 245279 \\
AFLOW-OQMD & \ce{Yb6Fe23} & $2.48$ & $53.27$ & $-50.79$ & 103706-634124-634132 \\
\midrule
MP-OQMD & \ce{Gd13Ge6O31F} & $91.00$ & $0.01$ & $90.99$ & 62329 \\
MP-OQMD & \ce{ZnFe16Ni7O32} & $38.00$ & $94.00$ & $-56.00$ & 182238 \\
MP-OQMD & \ce{Eu7Au3} & $50.72$ & $0.01$ & $50.71$ & 611842 \\
MP-OQMD & \ce{Gd6Zn23} & $42.88$ & $0.01$ & $42.87$ & 636504 \\
MP-OQMD & \ce{Gd6C3Cl5} & $42.69$ & $0.00$ & $42.68$ & 202547 \\
MP-OQMD & \ce{Gd10S19} & $42.00$ & $0.00$ & $42.00$ & 416804 \\
MP-OQMD & \ce{Gd6Mn23} & $57.76$ & $16.06$ & $41.70$ & 104076-635803-635804-635928-635948-635951-635954 \\
MP-OQMD & \ce{Ba8Eu7Cl34} & $45.00$ & $4.02$ & $40.98$ & 408479 \\
MP-OQMD & \ce{Mn9Au31} & $0.28$ & $39.05$ & $-38.77$ & 58552 \\
MP-OQMD & \ce{Eu5Pd2} & $36.02$ & $0.00$ & $36.02$ & 631525 \\
\bottomrule
\end{tabular}


==> multi-icsd-id-tables/outliers__volume_per_atom.tex <==
\begin{tabular}{l l r r r c}
\toprule
Databases & Composition & $V^1$ & $V^2$ & $\Delta^{1-2}$ & ICSD UID \\
 & & \multicolumn{3}{c}{(\AA$^3$/atom)} & \\
\midrule
AFLOW-MP & \ce{Bi} & $31.51$ & $103.72$ & $-72.21$ & 51675 \\
AFLOW-MP & \ce{MnNiAs} & $15.70$ & $84.29$ & $-68.59$ & 161716 \\
AFLOW-MP & \ce{Hg} & $28.86$ & $95.21$ & $-66.35$ & 79804 \\
AFLOW-MP & \ce{HoS} & $39.85$ & $103.31$ & $-63.46$ & 66357 \\
AFLOW-MP & \ce{SrPSe3} & $89.79$ & $27.94$ & $61.85$ & 412766 \\
AFLOW-MP & \ce{CsPbI3} & $91.23$ & $48.04$ & $43.20$ & 161480-250744-27979 \\
AFLOW-MP & \ce{NbTeBr3} & $75.01$ & $34.02$ & $40.99$ & 35376 \\
AFLOW-MP & \ce{N} & $47.65$ & $6.73$ & $40.92$ & 638342-644518 \\
AFLOW-MP & \ce{CeBr3} & $67.72$ & $31.52$ & $36.20$ & 31582 \\
AFLOW-MP & \ce{Se} & $63.04$ & $31.90$ & $31.14$ & 150731 \\
\midrule
AFLOW-OQMD & \ce{SrPSe3} & $89.79$ & $27.65$ & $62.14$ & 412766 \\
AFLOW-OQMD & \ce{CsPbI3} & $91.23$ & $46.85$ & $44.39$ & 161480-250744-27979 \\
AFLOW-OQMD & \ce{NbTeBr3} & $75.01$ & $30.71$ & $44.30$ & 35376 \\
AFLOW-OQMD & \ce{N} & $47.65$ & $7.39$ & $40.26$ & 638342-644518 \\
AFLOW-OQMD & \ce{CeBr3} & $67.72$ & $31.01$ & $36.71$ & 31582 \\
AFLOW-OQMD & \ce{H} & $37.20$ & $2.73$ & $34.47$ & 28465 \\
AFLOW-OQMD & \ce{CsTl} & $14.22$ & $47.71$ & $-33.49$ & 165344 \\
AFLOW-OQMD & \ce{Se} & $63.04$ & $31.39$ & $31.65$ & 150731 \\
AFLOW-OQMD & \ce{FeSeBr7} & $66.74$ & $37.22$ & $29.52$ & 39528 \\
AFLOW-OQMD & \ce{CaPSe3} & $53.48$ & $25.50$ & $27.98$ & 412765 \\
\midrule
MP-OQMD & \ce{Bi} & $103.72$ & $31.53$ & $72.20$ & 51675 \\
MP-OQMD & \ce{MnNiAs} & $84.29$ & $14.74$ & $69.55$ & 161716 \\
MP-OQMD & \ce{Hg} & $95.21$ & $27.10$ & $68.11$ & 79804 \\
MP-OQMD & \ce{CoO2} & $57.55$ & $11.71$ & $45.84$ & 89837 \\
MP-OQMD & \ce{H2} & $41.87$ & $3.33$ & $38.53$ & 28339-56055-638165-638168-638170-68271-94310-94311 \\
MP-OQMD & \ce{Cd6Sb5} & $62.94$ & $31.30$ & $31.65$ & 52832 \\
MP-OQMD & \ce{Cl2} & $70.98$ & $41.47$ & $29.50$ & 22406 \\
MP-OQMD & \ce{LiBH4} & $37.31$ & $9.87$ & $27.44$ & 168803 \\
MP-OQMD & \ce{HfPd5} & $41.53$ & $15.69$ & $25.84$ & 168289 \\
MP-OQMD & \ce{Kr} & $68.54$ & $42.83$ & $25.71$ & 426950-43726 \\
\bottomrule
\end{tabular}


==> multi-icsd-id-tables/unphys_props.tex <==
\begin{tabular}{l l r c}
\toprule
Database & Composition & Property value & ICSD UID \\
\midrule
\multicolumn{4}{c}{Formation Energy (eV/atom)} \\
AFLOW & \ce{SiO2} & $-11.950$ & 170547 \\
MP & \ce{Ta} & $5.113$ & 54207 \\
OQMD & \ce{CuO2} & $1126.321$ & 54126 \\
OQMD & \ce{SiO2} & $84.972$ & 155252 \\
OQMD & \ce{U6Ni} & $20.840$ & 105435-260983-647009 \\
OQMD & \ce{Sc5Ga3} & $8.575$ & 165189 \\
\midrule
\multicolumn{4}{c}{Volume (\AA$^3$/atom)} \\
MP & \ce{HoVO4} & $364.707$ & 152694 \\
MP & \ce{HgH3IO6} & $188.228$ & 409499 \\
MP & \ce{Rb} & $523.351$ & 109016 \\
MP & \ce{CaC2} & $896.388$ & 252718 \\
MP & \ce{EuAg} & $962.227$ & 58257 \\
MP & \ce{SnSe} & $182.422$ & 52425 \\
MP & \ce{Na} & $349.842$ & 70067 \\
MP & \ce{TcB} & $733.428$ & 168896 \\
MP & \ce{K} & $433.990$ & 157565 \\
MP & \ce{TlCl2} & $386.012$ & 20762 \\
MP & \ce{Ta} & $309.658$ & 54207 \\
MP & \ce{Fe3C} & $217.282$ & 76827 \\
MP & \ce{Cu} & $603.475$ & 150682 \\
\bottomrule
\end{tabular}


==> multi-icsd-id-tables/within_db_comp_mm.tex <==
\begin{tabular}{l l c}
\toprule
Database & Compositions & ICSD UID \\
\midrule
AFLOW & \ce{Li2O}, \ce{LiO2} & 173180-173193-173206-180569-22402-54368-57411-60431-642216-642219 \\
AFLOW & \ce{W}, \ce{W3O} & 150496-52344 \\
AFLOW & \ce{YIO}, \ce{Ba2CeCl7}, \ce{Ba2LaCl7}, \ce{YBrO}, \ce{AgSbTe2}, \ce{Bi}, \ce{Ba2YCl7} & 0 \\
AFLOW & \ce{Cr2Te4O11}, \ce{LiB} & 1 \\
AFLOW & \ce{PbSe}, \ce{SeS} & 183008-186790-187699-238502-238609-248492-248493-290054-38294-53933-600252-600599-600730-603893-62195-62196-63096-63097-648512-648513-648515-648516-648517-648518-648519-648520-648521-648522-648524-648525-648527-648528-657561-76644 \\
AFLOW & \ce{YFe2}, \ce{AlFe2} & 103697-103698-106699-150744-57792-601992-603459-632228-632234-634075-634079-634083-634084-634085-634088-634091-634096-634097-634099-634100-634102-634103-634105-634106-634107-634108-634114-634117-634122 \\
AFLOW & \ce{V2H}, \ce{V} & 151408-171003-183412-260470-426983-43420-43619-43718-44322-44509-44873-52537-53792-60614-62131-653393-653394-653395-653398-653399-76167-76269 \\
AFLOW & \ce{AgSbTe2}, \ce{CeNi2} & 102228-102229-602020-603815-621589-621596-621601-621602-621604-621609-621611-621613-621616-621617-621621-621623-657904 \\
AFLOW & \ce{SrGaH5}, \ce{SrGaH4} & 240697 \\
AFLOW & \ce{BaGaH4}, \ce{BaGaH5} & 240693 \\
AFLOW & \ce{Ba2HN}, \ce{Ba2N} & 409851-411436-414328-67510 \\
AFLOW & \ce{KFeSe2}, \ce{KFeS2} & 632398-632405 \\
\midrule
OQMD & \ce{Li2O}, \ce{LiO2} & 173180-173193-173206-180569-22402-54368-57411-60431-642216-642219 \\
OQMD & \ce{W}, \ce{W3O} & 150496-52344 \\
OQMD & \ce{UW4C4}, \ce{UW2C2} & 39222-42959 \\
OQMD & \ce{YFe2}, \ce{AlFe2} & 103697-103698-106699-150744-57792-601992-603459-632228-632234-634075-634079-634083-634084-634085-634088-634091-634096-634097-634099-634100-634102-634103-634105-634106-634107-634108-634114-634117-634122 \\
OQMD & \ce{ZnCoCuAg}, \ce{LiMgSnPd} & 16478 \\
OQMD & \ce{PbSe}, \ce{SeS} & 183008-186790-187699-238502-238609-248492-248493-290054-38294-53933-600252-600599-600730-603893-62195-62196-63096-63097-648512-648513-648515-648516-648517-648518-648519-648520-648521-648522-648524-648525-648527-648528-657561-76644 \\
\bottomrule
\end{tabular}


==> sections/progpot.tex <==
Increasingly large quantities of materials data are being calculated from
scratch using methods such as high-throughput density functional theory (DFT).
Data from such high-throughput databases are routinely used in materials
informatics efforts to predict novel materials and their properties.
However, a combination of the large-scale, automated nature of these databases
and the numerous adjustable parameters, with several different but reasonable
choices, used in each calculation introduces fundamental uncertainties in the
properties calculated.
Here, we quantify such uncertainties by critically comparing three of the
largest high-throughput materials databases available.
The ``error bars'' derived here can boost the effectiveness of learning-based
approaches, and also shed light on the most important sources of uncertainty in
high-throughput DFT.
Our findings surrounding these underlying sources of uncertainty can guide the
development of next-generation computational databases with improved
reproducibility.

